Deep SDSS optical spectroscopy of distant halo stars I. Atmospheric parameters and stellar metallicity distribution

We analyze a sample of tens of thousands of spectra of halo turnoff stars, obtained with the optical spectrographs of the Sloan Digital Sky Survey (SDSS), to characterize the stellar halo population "in situ" out to a distance of a few tens of kpc from the Sun. In this paper we describe the derivation of atmospheric parameters. We also derive the overall stellar metallicity distribution based on F-type stars observed as flux calibrators for the Baryonic Oscillations Spectroscopic Survey (BOSS). Our analysis is based on an automated method that determines the set of parameters of a model atmosphere that reproduces each observed spectrum best. We used an optimization algorithm and evaluate model fluxes by means of interpolation in a precomputed grid. In our analysis, we account for the spectrograph's varying resolution as a function of fiber and wavelength. Our results for early SDSS (pre-BOSS upgrade) data compare well with those from the SEGUE Stellar Parameter Pipeline (SSPP), except for stars with logg (cgs units) lower than 2.5. An analysis of stars in the globular cluster M13 reveals a dependence of the inferred metallicity on surface gravity for stars with logg < 2.5, confirming the systematics identified in the comparison with the SSPP. We find that our metallicity estimates are significantly more precise than the SSPP results. We obtain a halo metallicity distribution that is narrower and more asymmetric than in previous studies. The lowest gravity stars in our sample, at tens of kpc from the Sun, indicate a shift of the metallicity distribution to lower abundances, consistent with what is expected from a dual halo system in the Milky Way.

==> ReadMe <==
AA/2014/24053       Deep SDSS Optical Spectroscopy       (Allende Prieto+, 2014)
================================================================================
Deep SDSS Optical Spectroscopy of Distant Halo Stars.
I. Atmospheric parameters and stellar metallicity distribution.
   Allende Prieto, C. et al.
   <Astron. Astrophys. xxx,yyy (2014)>
   =2014A&A...
================================================================================
ADC Keywords: Abundances, [Fe/H]
    Milky Way
    Models, atmosphere
    Spectroscopy
    Stars, F-type
    Stars, metal-deficient
    Surveys
Keywords: stars: abundances, fundamental parameters, population II ?
    Galaxy: stellar content, halo
    
Abstract: We analyze a sample of tens of thousands of spectra of
	halo turnoff stars, obtained with the optical spectrographs
	of the Sloan Digital Sky Survey (SDSS), 
	to characterize the  stellar halo population "in situ"
	out to a distance of a few tens of kpc from the Sun. In this paper we describe
	the derivation of atmospheric parameters. We also derive the overall stellar
	metallicity distribution based on F-type stars observed as flux calibrators
	for the Baryonic Oscillations Spectroscopic Survey (BOSS).
	Our analysis is based on an automated method that determines the set 
	of parameters of a model atmosphere that best reproduces each 
	observed spectrum. We use an optimization algorithm and evaluate
	model fluxes by means of interpolation in a pre-computed grid.  
	In our analysis, we account for the spectrograph's varying resolution 
	as a function of fiber and wavelength. Our results for early
	SDSS (pre-BOSS upgrade) data compare well with those from the 
	SEGUE Stellar Parameter Pipeline (SSPP), except for stars at $\log$ g (cgs units) 
	lower than 2.5. 
	An analysis of stars in the globular cluster M13 reveals a dependence of 
        the inferred metallicity on surface gravity for stars with $\log g < 2.5$, confirming
        the systematics identified in the comparison with the SSPP. We find that our metallicity 
        estimates  are significantly more precise than the SSPP results.
	We also find excellent agreement with several independent analyses.
	We show that the SDSS color criteria for 
	selecting F-type halo turnoff stars as flux calibrators 
	efficiently excludes stars with high metallicities, but does not significantly distort 
	the shape of the metallicity distribution at low
	metallicity. We obtain a halo metallicity distribution that is narrower
	and more asymmetric than in previous studies. The lowest gravity stars
	in our sample, at tens of kpc from the Sun, indicate a shift
	of the metallicity distribution to lower abundances, consistent with that 
	expected from a dual halo system in the Milky Way.


File Summary:
--------------------------------------------------------------------------------
 FileName   Lrecl  Records   Explanations
--------------------------------------------------------------------------------
ReadMe         80        .   This file
table1.dat     54     3808   Model SDSS ugriz colors
--------------------------------------------------------------------------------

Byte-by-byte Description of file: table1.dat
--------------------------------------------------------------------------------
   Bytes Format Units    Label  Explanations
--------------------------------------------------------------------------------
   1- 6   F6.2  ---      [Fe/H] Metallicity
   8- 15  I8     K       Teff   Effective temperature 
  17- 22  F6.2  ---      logg   log10 of the surface gravity (g in cgs units)
  24- 30  F7.3  mag      u-g    u-g color
  32- 38  F7.3  mag      g-r    g-r color
  40- 46  F7.3  mag      r-i    r-i color
  48- 54  F7.3  mag      i-z    i-z color
--------------------------------------------------------------------------------
Model SDSS colors for Kurucz model atmospheres.
--------------------------------------------------------------------------------
(End)       
